A Visual Attention Grounding Neural Model for Multimodal Machine Translation

We introduce a novel multimodal machine translation model that utilizes parallel visual and textual information. Our model jointly optimizes the learning of a shared visual-language embedding and a translator. The model leverages a visual attention grounding mechanism that links the visual semantics with the corresponding textual semantics. Our approach achieves competitive state-of-the-art results on the Multi30K and the Ambiguous COCO datasets. We also collected a new multilingual multimodal product description dataset to simulate a real-world international online shopping scenario. On this dataset, our visual attention grounding model outperforms other methods by a large margin.

==> table.tex <==
\begin{table*}[h]
\caption{Statistic of the IKEA dataset}
\begin{tabular}{lllll}
Pair       & EN-DE  &        & EN-FR  &        \\ \hline
Language   & EN     & DE     & EN     & FR     \\
Tokens     & 256355 & 216892 & 239966 & 275251 \\
Min length & 6      & 6      & 6      & 6      \\
Max length & 343    & 324    & 334    & 469    \\
Avg length & 71.4   & 60.4   & 72.2   & 82.9   \\
Std dev    & 46.3   & 39.1   & 47.2   & 54.7   \\
Vocabulary & 6601   & 10468  & 6442   & 7575  
\end{tabular}
\label{table:table_0}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{|c|p{5cm}|p{5cm}|}
\hline
Product Image & Source Description & Target Description \\
\hline
\raisebox{-\totalheight}{\includegraphics[width=0.2\textwidth, height=40mm]{4634.jpg}} & the 4 large drawers on casters give you an extra storage space under the bed . adjustable bed sides allow you to use mattresses of different thicknesses . 17 slats of layer glued birch adjust to your body weight and increase the suppleness of the mattress . wipe clean using a damp cloth and a mild cleaner . wipe dry with a clean cloth .
& die 4 geräumigen schubladen auf rollen sorgen für zusätzlichen stauraum unter dem bett . durch verstellbare bettseiten können matratzen in verschiedenen stärken verwendet werden . mit feuchtem tuch ( evtl . mit mildem reinigungsmittel ) abwischen . mit trockenem tuch nachwischen .
\\
\hline
\end{tabular}
\caption{An example of product description and the corresponding translation in German from the \textbf{IKEA dataset}. Both description provide an accurate caption of the commercial characteristics of product in the image, but the details in the descriptions are different.}
\label{table:table_5}
\end{table*}
